TADM: Temporally-Aware Diffusion Model for Neurodegenerative Progression on Brain MRI

Generating realistic images to accurately predict changes in the structure of brain MRI is a crucial tool for clinicians. Such applications help assess patients' outcomes and analyze how diseases progress at the individual level. However, existing methods for this task present some limitations. Some approaches attempt to model the distribution of MRI scans directly by conditioning the model on patients' ages, but they fail to explicitly capture the relationship between structural changes in the brain and time intervals, especially on age-unbalanced datasets. Other approaches simply rely on interpolation between scans, which limits their clinical application as they do not predict future MRIs. To address these challenges, we propose a Temporally-Aware Diffusion Model (TADM), which introduces a novel approach to accurately infer progression in brain MRIs. TADM learns the distribution of structural changes in terms of intensity differences between scans and combines the prediction of these changes with the initial baseline scans to generate future MRIs. Furthermore, during training, we propose to leverage a pre-trained Brain-Age Estimator (BAE) to refine the model's training process, enhancing its ability to produce accurate MRIs that match the expected age gap between baseline and generated scans. Our assessment, conducted on the OASIS-3 dataset, uses similarity metrics and region sizes computed by comparing predicted and real follow-up scans on 3 relevant brain regions. TADM achieves large improvements over existing approaches, with an average decrease of 24% in region size error and an improvement of 4% in similarity metrics. These evaluations demonstrate the improvement of our model in mimicking temporal brain neurodegenerative progression compared to existing methods. Our approach will benefit applications, such as predicting patient outcomes or improving treatments for patients.

==> Tmp/01_template.tex <==
\subsection{A Subsection Sample}
Please note that the first paragraph of a section or subsection is
not indented. The first paragraph that follows a table, figure,
equation etc. does not need an indent, either.

Subsequent paragraphs, however, are indented.

\subsubsection{Sample Heading (Third Level)} Only two levels of
headings should be numbered. Lower level headings remain unnumbered;
they are formatted as run-in headings.

\paragraph{Sample Heading (Fourth Level)}
The contribution should contain no more than four levels of
headings. Table~\ref{tab1} gives a summary of all heading levels.

\begin{table}
\caption{Table captions should be placed above the
tables.}\label{tab1}
\begin{tabular}{|l|l|l|}
\hline
Heading level &  Example & Font size and style\\
\hline
Title (centered) &  {\Large\bfseries Lecture Notes} & 14 point, bold\\
1st-level heading &  {\large\bfseries 1 Introduction} & 12 point, bold\\
2nd-level heading & {\bfseries 2.1 Printing Area} & 10 point, bold\\
3rd-level heading & {\bfseries Run-in Heading in Bold.} Text follows & 10 point, bold\\
4th-level heading & {\itshape Lowest Level Heading.} Text follows & 10 point, italic\\
\hline
\end{tabular}
\end{table}


\noindent Displayed equations are centered and set on a separate
line.
\begin{equation}
x + y = z
\end{equation}
Please try to avoid rasterized images for line-art diagrams and
schemas. Whenever possible, use vector graphics instead (see
Fig.~\ref{fig1}).

\begin{figure}
\includegraphics[width=\textwidth]{figures/fig1.eps}
\caption{A figure caption is always placed below the illustration.
Please note that short captions are centered, while long ones are
justified by the macro package automatically.} \label{fig1}
\end{figure}

\begin{theorem}
This is a sample theorem. The run-in heading is set in bold, while
the following text appears in italics. Definitions, lemmas,
propositions, and corollaries are styled the same way.
\end{theorem}
%
% the environments 'definition', 'lemma', 'proposition', 'corollary',
% 'remark', and 'example' are defined in the LLNCS documentclass as well.
%
\begin{proof}
Proofs, examples, and remarks have the initial word in italics,
while the following text appears in normal font.
\end{proof}
For citations of references, we prefer the use of square brackets
and consecutive numbers. Citations using labels or the author/year
convention are also acceptable. The following bibliography provides
a sample reference list with entries for journal \cite{lam2000mathematical}
%articles~\cite{ref_article1}, an LNCS chapter~\cite{ref_lncs1}, a
%book~\cite{ref_book1}, proceedings without editors~\cite{ref_proc1},
%and a homepage~\cite{ref_url1}. Multiple citations are grouped
%\cite{ref_article1,ref_lncs1,ref_book1},
%\cite{ref_article1,ref_book1,ref_proc1,ref_url1}.

==> Tmp/3_proposed_method_old.tex <==
\mypar{Denoising Diffusion Probabilistic Models}
DDPM \cite{ho2020denoising} are generative models that learn a Markov chain process to convert the Gaussian distribution into the data distribution. During the diffusion process, Gaussian noise is added in successive steps to a sample $x_0$ from the given data distribution $q(x_0)$, to convert it into a latent variable distribution $q(x_t)$, as follows:

\begin{equation}
    q(x_{1},x_{2},\dots,x_{T}|x_{0}) = \prod_{t=1}^{T}q(x_{t}|x_{t-1})
\end{equation}
%with
\begin{equation}
    q(x_{t}|x_{t-1})= \mathcal{N}(x_{t};\sqrt{1-\beta_{t}}x_{t-1},\beta_{t}\textbf{I})
\end{equation}
where $t \in {1, . . . , T}$ is the diffusion step, $\mathcal{N}$ represents the Gaussian distribution, $\beta_{t}$ is a noise variance , and $\textbf{I}$ is the identity matrix.

Then, during the reverse process, the latent variable distribution $p_{\theta}(x_{t})$ is transformed progressively into the data distribution $p_{\theta}(x_{0})$, which is parameterized by $\theta$, by letting the model learn the following Gaussian transformations:
\begin{equation}
    p_{\theta}(x_{0},x_{1},\dots,x_{T-1}|x_{T}) = \prod_{t=1}^{T}p_{\theta}(x_{t-1}|x_{t})
\end{equation}
%with 
\begin{equation}
    p_{\theta}(x_{t-1}|x_{t})= \mathcal{N}(x_{t-1};\mu_{0}(x_{t},t),\sigma_{0}(x_{t},t)^{2}\textbf{I})
\end{equation}
\begin{equation}
    p(x_t)= \mathcal{N}(x_T; \textbf{0}, \textbf{I})
\end{equation}

where $\mu_{0}(x_{t},t)$ represents the mean of the Gaussian distribution at the $t$ reverse step, and $,\sigma_{0}(x_{t},t)^{2}$ denotes the variance of the Gaussian distribution at the $t$ reverse step.
+++ADD DIFFUSION LOSS?+++




%Inflammation (infection, demyelination) is described by dark in T1-w


%The general structure of the proposed method, TADM, is depicted in Fig.\ref{fig:network}. Our model, built for source $S$ and target $G$, consists of a diffusion module with the integration of a temporal-regressor component. As the diffusion module infers the latent code, the temporal-regressor dynamically adapts the loss function to correct the generated output, ultimately increasing the overall versatility of the pipeline  compared to direct conditioning approaches.

%\subsection{Dataset Details}
%\label{sec:dataset}
%\input{4_dataset_details}

\subsection{Problem Formulation}
This work addresses the brain progression modelling task on brain MRI scans. Let $\mathbf{I}^P_{T_1} \in \mathbb{R}^{H \times W}$ and $\mathbf{I}^P_{T_2} \in \mathbb{R}^{H \times W}$ be two MRI scans acquired on the patient $P$ during two different medical session occurred at timepoints $T_1$ and $T_2$, respectively. For semplicity, we omit the superscript $P$ in the following. We define the \textit{temporal gap} $\Delta_{1,2} = T_2-T_1$ as the number of months passed between the acquisition of the two MRI's. Values of temporal gaps in the dataset can vary from few months to several years. Let also be $A$ and $BCS$ the age and the brain cognitive status  of the patient at the moment of the acquisition. The brain cognitive status $BCS \in {0,1,2}$ is a categorical variable that describe the cognitive status of the patients classifying it into three categories: $0$ for normal patients, $1$ for patients affected by light neurodegeneration, $2$ for patients affected by serious neurodegeneration.
During the training, a deep generative model $G_\theta$, parametrized by $\theta$, is trained to receive as input the previous scan $\mathbf{I}_{T_1}$ and predict $\mathbf{\hat{I}}_{T_2} = G_\theta(\mathbf{I}_{T_1})$, to reconstruct the latest scan $\mathbf{I}_{T_2}$. At inference time, the model should generate $\mathbf{\hat{I}}_{T_N} = G_\theta(\mathbf{I}_{T_1})$ corresponding to an arbitrarily future timepoint $T_N$, receiving as input $\mathbf{I}_{T_1}$.

\subsection{Conditional Diffusion Model for Future Brain MRIs Generation}
We leveraged a DDPM to generate realistic brain MRI's at an arbitrarily future timepoint $T_x$. We aim at learning how brain structures changes over time to model the brain progression. To enforce this, the diffusion model is trained to produce residual images that are then added to the input $I_{T_a}$ given as an input. This means that our DDPM estimates the pixel-wise difference $\mathbf{\bar{I}}_{\Delta_{a,b}} = \mathbf{I}_{T_b} - \mathbf{I}_{T_a}$, given $\mathbf{I}_{T_a}$ as an input and $\mathbf{I}_{T_b}$ as future scan to be predicted.
%During the diffusion process, given a pair of MRIs $\mathbf{I}_{T_1}$ and $\mathbf{I}_{T_2}$, we compute their residual image $\mathbf{\bar{I}}_{\Delta_{1,2}} = \mathbf{I}_{T_2} - \mathbf{I}_{T_1}$ as the pixel-wise difference between the two scans. 
The residual image $\mathbf{\bar{I}}_{\Delta_{1,2}}$ is then used as input for the diffusion process, \textit{i.e.} $x_0 = \mathbf{\bar{I}}_{\Delta_{a,b}}$ (\textit{c.f.} \Cref{sec:rel_works}). Note that we associate the temporal gap $\Delta_{a,b}$ as metadata on the residual image, as it represents the amount of time lapsed between two scans. %to observe the changes in the brain visible in $\mathbf{\bar{I}}_{\Delta_{1,2}}$.

To train $G_\theta$ to generate a residual image for a specific input scan $\mathbf{I}_{T_a}$, the diffusion model is conditioned with features extracted on $\mathbf{I}_{T_a}$ by an encoder $\phi$ based on Residual-in-Residual Dense Blocks (RRDB) \cite{RRDB}. The conditioning is performed by fusing the features obtained by $\phi$ with the activation map of the first convolutional block of the diffusion model. During the reverse process, the diffusion model generates an MRI at an arbitrarily future timepoint $T_x$, given an input scan $\mathbf{I}_{T_a}$. The model is conditioned on $\mathbf{I}_{T_a}$ to progressively denoise the Gaussian Noise variable $X_T$ and predict the residual image $\mathbf{\hat{I}}_{\Delta_{a,x}}$, where $\Delta_{a,x} = T_x - T_a$ is the desired residual image representing the temporal gap of structural changes between the input and the generated MRI scans. Finally, the generated brain MRI $\mathbf{I}_{T_x} = \mathbf{I}_{T_a} + \mathbf{\hat{I}}_{\Delta_{a,x}}$ is obtained by adding the predicted residual image to the input.

At this point, our model is not aware of the temporal gap between current and future scans. We will introduce the temporally-aware component of our model over the next sections.

\subsection{Learning the Temporal Evolution in Brain MRI scans}
\label{sec:conditioning}
% Previous state-of-the-art methods \cite{ravi2019degenerative,SADM,DDM}, used age conditioning during training to learn the correlation between ages and brain MRI's. During inference, ages was instead used to codify the desired future timepoint $T_N$.
% However, using only age conditioning the model is not explicitly trained to learn the relationship between the temporal gap among the acquisition of the two MRI's and the anatomical changes occurred during that period of time. Moreover, this strategy requires that the ages are equally and homogeneously represented in the training set. If the training set does not contain any (or enough) sample acquired at a specific age, the model will not be able to generate MRI's at that age. However, this requirement is rarely satisfied in real world datasets.

Differently than the current state-of-the-art \cite{DDM,ravi2019degenerative,SADM}, we condition the model with the temporal gap $\Delta_{a,b}$, by encoding the amount of time lapsed between two MRI's. By doing so, the model is encouraged to learn the underlying relationship between the structural changes observed in the MRI's and their time interval. Conditioning with the temporal gap is crucial to enable the model to learn and predict the evolution of a neurodegeneration over time, which requires to understand structural changes occurring in a define time interval.

Moreover, to leverage additional information useful for the generation of more accurate and personalised MRI's, we 
provide the model with additional metadata of the input $\mathbf{I}_{T_a}$ (if any). Particularly, the metadata consists in the age $A$ and the brain cognitive status $BCS$ at the moment of the acquisition of $\mathbf{I}_{T_a}$. It is important to note that the metadata $A$ used in our model refers to the input image, and not to the desired output $\mathbf{\hat{I}}_{T_b}$, as the state-of-the-art currently do \cite{DDM,ravi2019degenerative,SADM}. Similar to \cite{diffusion_model1}, metadata is encoded using the Transformer sinusoidal positional embedding \cite{transformer} before being provided into the model.

The strategy of using the temporal gap in our training has two main advantages: (i) it allows the generation of a scan with an arbitrarily temporal gap $\Delta_{a,x}$ with respect to $\mathbf{I}_{T_a}$; (ii), it encourage the model to learn how the brain changes over that time interval. However, the conditioning only occurs at the feature level, which implies that it does not directly guide the generation process. This means there is guarantee that the generated structural changes on the brain are coherent with the temporal gap $\Delta_{a,x}$ of a given patients. We overcome this shortcoming by introducing a novel \textit{Temporal Gap Estimator} (TGE) to the training process, which details are provided in the following section.
%Note that differently from previous works, $A$ is not the age of the patient at the future timepoint $T_N$, but it is the age of the patient at the timepoint $T_1$ used to guide the generation process.
%Note that differently from previous works, $A$ is the age of the patient at the timepoint $T_1$ rather than the age at the future timepoint $T_N$.

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\linewidth]{figures/pipeline.pdf}
%\caption{\color{red}Pipeline of the model at training time. In the first row the diffusion process is performed starting from the difference of pair $D$. The second row shoes the reverse process with the latent varible $D_{t}$ denoised through the Conditional Noise Predictor $P$.}
%    \label{fig:network}
%\end{figure}


\begin{figure}[t]
        \centering
        \includegraphics[width=\linewidth]{figures/fig1.png}
    \caption{The \textit{Temporally-Aware Diffusion Model} (TADM) comprises three main parts (surrounded by coloured dashed boxes). \textsc{\color{red}red:} The DDPM takes a residual image, calculated as the difference between two scans acquired at two the time points $T_a$ and $T_b$, on which random noise $\epsilon$ is applied. The DDPM is trained to denoise the residual image through several diffusion steps. The denoised residual image $\hat{I}_{\Delta_{a,b}}$ and the scan $I_{T_a}$ are summed together to estimate the scan $\hat{I}_{T_b}$ at time $T_{b}$. \textsc{\color{blue}blue:} Here, we encode the scan $I_{T_a}$ to extract a representation $z_a$ used to condition the DDPM, in conjunction with the brain condition score and the patient's age at time $T_a$. \textsc{\color{mygreen}green:} The estimated $\hat{I}_{T_b}$ is provided to the encoder to extract the features $z_b$ that, together with the previously extracted features $z_a$, are provided as inputs to the \textit{Temporal Gap Estimator} (TGE) to predict the time interval $\hat{\Delta}_{a,b}$. The \textsc{snowflake} indicates model with frozen parameters.}
    \label{fig:pipeline}
    \end{figure}

%\subsection{Diffusion Model} 

%In this section, we aim to offer a foundational comprehension of a diffusion model (DDPM). Introduce by \cite{ho2020denoising} DDPM  represent a type of generative model that employs a Markov chain to systematically introduce noise to a given data distribution $q(x_0)$ of input $x_0$, subsequently converting it into a latent variable $q(x_t)$ through an iterative diffusion procedure that follow:
%\begin{equation}
%    q(x_{1},x_{2},\dots,x_{T}|x_{0}) = \prod_{t=1}^{T}q(x_{t}|x_{t-1})
%\end{equation}
%with
%\begin{equation}
%    q(x_{t}|x_{t-1})= \mathcal{N}(x_{t};\sqrt{1-\beta_{t}}x_{t-1},\beta_{t}I)
%\end{equation}
%where $\mathcal{N}$ represents the Gaussian distribution, $\beta_{t}$ is a noise variance , and $I$ is a matrix of ones.
%Employing a reverse process, the latent variable distribution
%$p_{\theta}(x_{t})$ is transformed progressively 
%into the data distribution $p_{\theta}(x_{0})$, which is parameterized by $\theta$,
%by letting the model learn
% the following Gaussian transformations:
%\begin{equation}
%    p_{\theta}(x_{0},x_{1},\dots,x_{T-1}|x_{T}) = \prod_{t=1}^{T}p_{\theta}(x_{t-1}|x_{t})
%\end{equation}
%with 
%\begin{equation}
%    p_{\theta}(x_{t-1}|x_{t})= \mathcal{N}(x_{t-1};\mu_{0}(x_{t},t),\sigma_{0}(x_{t},t)^{2}I)
%\end{equation}

%where $\mu_{0}(x_{t},t)$ represents the mean of the Gaussian distribution at the $t$ reverse step, and $,\sigma_{0}(x_{t},t)^{2}$ denotes the variance of the Gaussian distribution at the $t$ reverse step. The objective of our method is to obtain a model able to take an input T1w at time $t_{1}$ ($I_{t1}$ in the following) and generate T1w at time $t_{2}$  ($I_{t2}$ in the following). The employing  of DDPM was done exploiting the idea of \cite{li2022srdiff}: rather than directly generating $I_{t2}$, we opt for residual prediction to produce the difference $D$ between $I_{t2}$ and $I_{t1}$. 

%The diffusion process converts $D$ in a latent variable $D_{T}$ adding noise progressively, while the reverse process transforms $D_{T}$ in a residual image $D_{g}$ through iterative denoising; the last denoising step is conditioned by an encoder of $I_{t1}$. By adding $D_{g}$ to the input $I_{t1}$ the desired $I_{t2}$ must be generated. 

%\subsubsection{Training time} During the training step (see Fig.\ref{fig:network}) samples consist of pairs \{$I_{t1}$/$I_{t2}$\} and the parameter $T$ (number of diffusion steps) were used as input.
%For each pair, starting from the difference image $D$, the diffusion process adds Gaussian noise to $D$ to produce $D_{T}$.
%In the reverse process, $I_{t1}$ is encoded in $E_{t1}$ through a CNN based on Residual-in-Residual Dense Blocks (RRDB), and it is used for condition the denoising step, which starts from $D_{T}$ and samples the noise $\epsilon$ for each timestamp $t\in{1,\dots,T}$. The last step permits to train the conditional noise predictor $P$, which is basically a U-net.

%\subsubsection{Conditioning} The strategy to generate the residual image $D_{p}$ requires the use of conditioning through  $I_{t1}$. In order to better control the process other conditioning was added; specifically, during the reverse process, the age of the patient at time $t2$, the time distance in months between $t1$ and $t2$ and the disease progression (encoded by a number in the range [1,4]) were added. 

%\subsubsection{Inference time} The inference step takes the input $I_{t1}$ and its encoder $E_{t1}$, the number of diffusion steps $T$ and the conditional noise predictor $P$. First, $I_{t1}$ is encoded by $E_{t1}$ and the latent variable $D_{T}$ is generated from the standard Gaussian distribution, then for each step $t=T,T-1,\dots,1$, the denoised $D_{t}$ is performed using $P$. At $t=1$ the last denoising step is performed, and the residual image $D_{p}$ is generated. 



\subsection{Brain-Age Gap Estimator}
\label{sec:tge}
The strategy described in \cref{sec:conditioning} has two main advantages: firstly, it allows the generation of scan with arbitrarily temporal gap $\Delta_{1,N}$ with respect $\mathbf{I}_{T_1}$; secondly, it encourage the model to learn how the brain has changed in that period of time.
Nonetheless, the conditioning only acts at the feature level, which implies that it does not directly guide the generation process.
Hence, this strategy does not ensure that the generated anatomical changes on the brain are coherent with the temporal gap $\Delta_{1,N}$.
%to ensure that generated MRI is coherent with the temporal gap $\Delta_{1,N}$.
%In other words, we need a strategy to ensures that the generated anatomical changes on the brain can be naturally occur in the amount of time defined by $\Delta_{1,N}$.
To solve this issue, we propose a novel strategy based on an auxiliary neural network, named \textit{Temporal Gap Estimator} (TGE). Integrated in the training of the diffusion model, the role of this model is to estimate the temporal gap between the input and the generated MRIs and to correct the generation process, when the estimated temporal gap is not in compliance with the desired gap $\Delta_{1,N}$.

The TGE model is firstly pretrained on pairs of MRIs from the training set to estimate their temporal gap. Formally, given two MRIs $\mathbf{I}_{T_1}$ and $\mathbf{I}_{T_b}$, and their temporal gap $\Delta_{a,b}$, we obtain their representations using the RRDB encoder. These two representation $z_a = \phi(\mathbf{I}_{T_a})$ and $z_b = \phi(\mathbf{I}_{T_b})$ are then provided to the TGE as an input. The estimated temporal gap $\widehat{\Delta}_{a,b} = TGE(z_a, z_b)$ is supervised by a standard \textit{Mean Squared Error} (MSE) loss between the estimated $\widehat{\Delta}_{1,2}$ and the real $\Delta_{1,2}$ temporal gaps.
%as follows:
%\begin{equation}
%    \mathcal{L}^{TGE}(\widehat{\Delta}_{1,2}, \Delta_{1,2}) = (\widehat{\Delta}_{1,2} - \Delta_{1,2})^2
%\end{equation}

After the pretraining, the parameters of the TGE model are frozen and used during the diffusion model training to steer the generation process, by estimating the temporal gap between the input and the generated MRIs. The error between the estimated and the desired gap will be backpropagated to the diffusion model to improve the generation process.

\subsection{Overall Framework}
In this section, we will provide a complete overview of the framework. \\
\textbf{Training}. We provide pairs of MRI scans $\mathbf{I}_{T_a}$ and $\mathbf{I}_{T_b}$ taken from a patient $P$ to condition the Diffusion Model $G_\theta$. The DDPM is trained to predict the artificial noise added during the diffusion process, by minimising the following objective:
\begin{equation}
    \label{eq:dml}
    \mathcal{L}^{DML} = \mathbb{E}_{\epsilon \sim \mathcal{N}(0,1), \mathbf{\bar{I}}_{\Delta_{a,b}}, \tau} \left[||G_\theta( \mathbf{\bar{I}}_{\Delta_{a,b}}, \tau; z_a, \Delta_{a,b}, A, BCS) - \epsilon ||^2_2 \right]
\end{equation}

\noindent where $\mathbf{\bar{I}}_{\Delta_{a,b}}$ is the residual image, $\tau$ is the diffusion timestep, $z_a$ is the encoded representation of the input scan $\mathbf{I}_{T_a}$, $\Delta_{a,b}$, $A$, and $BCS$ are the temporal gap, the age, and the brain cognitive status of the patient, respectively. Note that $z_a$, $\Delta_{a,b}$, $A$, and $BCS$ are used to condition the generation process.

%Moreover, at each diffusion step $t$, the predicted residual image $\mathbf{\hat{I}}_{\Delta_{1,2}}$ is obtained by removing the noise predicted by $G_\theta$. Accordingly, the reconstructed latest MRI $\mathbf{I}_{T_2} = \mathbf{I}_{T_1} + \mathbf{\hat{I}}_{\Delta_{1,2}}$ can be easily obtained by adding the predicted residual image to the previous MRI. 
%Moreover, at each diffusion step $\tau$, the reconstructed MRI $\mathbf{I}_{T_2} = \mathbf{I}_{T_1} + \mathbf{\hat{I}}_{\Delta_{1,2}}$ can be easily obtained by adding the previous MRI to the predicted residual image $\mathbf{\hat{I}}_{\Delta_{1,2}}$, which is produced by removing the noise predicted by $G_\theta$.
%Since the predicted $\mathbf{\hat{I}}_{T_2}$ reconstructs $\mathbf{I}_{T_2}$, the temporal gap between $\mathbf{\hat{I}}_{T_2}$ and $\mathbf{\hat{I}}_{T_1}$ should match the actual gap between the $\mathbf{I}_{T_1}$ and $\mathbf{I}_{T_2}$. If not, the generation should be corrected accordingly.
To steer the generation process, we use the pre-trained and frozen TGE model to estimate the temporal gap $\widehat{\Delta}_{a,b} = \operatorname{TGE}(z_a, \hat{z}_b)$, where $\hat{z}_b$ are the features extracted from the recostructed MRI image at time $T_b$ using the encode $\Phi$, \textit{i.e.} $\hat{z}_b = \phi(\hat{I}_{T_b})$, and $\hat{I}_{T_b}$ is obtained from the predicted residual image as described in \Cref{sec:conditioning}. We then optimise the following loss for the TGE:
\begin{equation}
    \label{eq:tge}
    \mathcal{L}^{TGE}(\widehat{\Delta}_{1,2}, \Delta_{1,2}) = (\widehat{\Delta}_{1,2} - \Delta_{1,2})^2
\end{equation}
Note that the gradients of this loss only update the diffusion model $G_\theta$ that produces the residual $\mathbf{\hat{I}}_{\Delta_{a,b}}$, as TGE parameters are frozen at this stage of the training.%which is used to calculate $\widehat{\Delta}_{1,2}$. The TGE model is freezed and will not optimised by this loss.

Finally, the overall loss is obtained by combining \cref{eq:dml,eq:tge} as follows:
\begin{equation}
    \mathcal{L}^{Tot} = \mathcal{L}^{DML} + \mathcal{L}^{TGE}
\end{equation}

\noindent \textbf{Inference}. The model receives an input MRI $\mathbf{I}_{T_a}$ and generates a future MRI with an arbitrarily temporal gap $\Delta_{a,x}$ with respect to the input. The reverse process starts from a Gaussian noise variable $X_T$ that is progressively denoised through $G_\theta( X_\tau, \tau; z_a, \Delta_{a,x}, A, BCS)$.%, where $t$ is the denoising timestep, $z_1 = \phi(\mathbf{I}_{T_1})$ is the encoded representation of $\mathbf{I}_{T_1}$ and $\Delta_{1,N}$, $A$, $BCS$ are the temporal gap, the age and the brain cognitive status, respectively. 
The predicted residual image  $\mathbf{\hat{I}}_{\Delta_{1,N}}$ is then added to the input MRI to generate the predicted future MRI (\textit{c.f.} \Cref{sec:conditioning}). %$\mathbf{\hat{I}}_{T_N} = \mathbf{I}_{T_1} + \mathbf{\hat{I}}_{\Delta_{1,N}}$.

==> Tmp/4_dataset_details.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}{1.06\textwidth}

        \begin{subfigure}{.237\textwidth}
          \centering
          \includegraphics[width=1.05\linewidth]{figures/t1.jpg}
          \caption{}
          \label{fig:t1}
        \end{subfigure}%
        \begin{subfigure}{.237\textwidth}
          \centering
          \includegraphics[width=1.05\linewidth]{figures/t2.jpg}
          \caption{}
          \label{fig:t2}
        \end{subfigure}
        \begin{subfigure}{.23\textwidth}
          \centering
          \includegraphics[width=1.045\linewidth]{figures/flair.jpg}
          \caption{}
          \label{fig:flair}
        \end{subfigure}
        \begin{subfigure}{0.221\textwidth}

          \centering
          \includegraphics[width=\linewidth]{figures/skull_removal.png}
          \caption{}
          \label{fig:skull_removal}
        
  
\end{subfigure}%
  
\end{subfigure}%



\caption{Example of a sequences: T1-weighted (a) T2-weighted (b) and Flair (c). Example of central slice T1-weighted from OASIS-3 after registration with MNI152 T1 1mm template and skull removal.}
\label{fig:sequences}
\end{figure*}

Our study starts from dataset OASIS-3~\cite{lamontagne2019oasis}, a retrospective dataset of $1378$ participants with acquisitions collected across several ongoing projects over the course of $30$ years. OASIS-3 is composed of $755$ cognitively normal adults and $622$ individuals at various stages of cognitive decline, aged between $42$ and $95$ years. The dataset encompasses $2842$ MR sessions, featuring T1w, T2w, FLAIR, ASL, SWI, time of flight, resting-state BOLD, and DTI sequences. Additional information such as the date of scan, the age of the patients and the state of patients complete the dataset.

Starting from the aforementioned dataset, a sub-dataset has been properly extracted. Firstly, only the Magnetic Resonance Images (MRI) were considered; in particular, we pay attention to the T1-weighted (T1-w) images, which are the MRI sequences generated by using short TE (Time to Echo) and TR (Repetition Time) times during the magnetization process. We chose to use this sequence because OASIS-3 is composed of normal ageing patients and Alzheimer's disease patients; in most cases, both conditions cause slow changes in the brain, then a more controlled contrast such as in T1-w (see Fig.~\ref{fig:sequences}) should help the model.

As explained in Section~\ref{sec:prop_meth} our approach is based on pairs of scans while in OASIS-3 some patients present a unique acquisition becoming unusable for our purpose, then $693$ patients were excluded remaining in $685$. From them, some patients have $2$ scans generating $2$ pairs, others have $9$ scans which generate $36$ different pairs. Since it is well known that MRIs from different devices produce different results, each scan of the selected patient was previously registered through the MNI152 template (T1-w, 1mm) and then visually verified: for each scan, the registered central slice was extracted and converted to a png file, and those that did not correspond to the same point in the brain were excluded from the dataset. At the end of this process, our subdataset is composed of $634$ different patients and $2535$ pairs of MRI saved with a label representing the number of day between them. During the registration step we made use of FSL library tools~\cite{jenkinson2012fsl}: specifically every scan was firstly registered through the command \textit{flirt} and then the skull was removed through the command \textit{bet} producing an output as in Fig.~\ref{fig:skull_removal}.
